Are we using appropriate segmentation metrics? Identifying correlates of human expert perception for CNN training beyond rolling the DICE coefficient

Metrics optimized in complex machine learning tasks are often selected in an ad-hoc manner. It is unknown how they align with human expert perception. We explore the correlations between established quantitative segmentation quality metrics and qualitative evaluations by professionally trained human raters. Therefore, we conduct psychophysical experiments for two complex biomedical semantic segmentation problems. We discover that current standard metrics and loss functions correlate only moderately with the segmentation quality assessment of experts. Importantly, this effect is particularly pronounced for clinically relevant structures, such as the enhancing tumor compartment of glioma in brain magnetic resonance and grey matter in ultrasound imaging. It is often unclear how to optimize abstract metrics, such as human expert perception, in convolutional neural network (CNN) training. To cope with this challenge, we propose a novel strategy employing techniques of classical statistics to create complementary compound loss functions to better approximate human expert perception. Across all rating experiments, human experts consistently scored computer-generated segmentations better than the human-curated reference labels. Our results, therefore, strongly question many current practices in medical image segmentation and provide meaningful cues for future research.

==> flow/front/00_authors_broken.tex <==
\author{%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\name Florian Kofler \\
	\addr
	Department of Informatics, Technical University Munich, Germany \\
	%
	\addr 
	TranslaTUM - Central Institute for Translational Cancer Research, Technical University of Munich, Germany \\
	%
	\addr
	Department of Diagnostic and Interventional Neuroradiology, School of Medicine, Klinikum rechts der Isar, Technical University of Munich, Germany
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\AND
	\name Ivan Ezhov \\
	\addr
	Department of Informatics, Technical University Munich, Germany \\
	% 
	\addr 
	TranslaTUM - Central Institute for Translational Cancer Research, Technical University of Munich, Germany
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\AND
	\name Fabian Isensee \\
	\addr
	Applied Computer Vision Lab, Helmholtz Imaging \\
	%
	\addr 
	Division of Medical Image Computing, German Cancer Research Center (DKFZ), Germany
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\AND
	\name Fabian Balsiger \\
	\addr
	Support Center for Advanced Neuroimaging (SCAN), Institute for Diagnostic and Interventional Neuroradiology, Inselspital, Bern University Hospital, University of Bern, Bern, Switzerland	%
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\AND
	\name Christoph Berger \\
	\addr
	Department of Informatics, Technical University Munich, Germany
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\AND
	\name Maximilian Koerner \\
	\addr
	Department of Informatics, Technical University Munich, Germany
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\AND
	\name Beatrice Demiray \\
	\addr
	Computer Aided Medical Procedures (CAMP), Technical University of Munich, Germany
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\AND
	\name Julia Rackerseder \\
	\addr
	Computer Aided Medical Procedures (CAMP), Technical University of Munich, Germany \\
	\addr
	ImFusion GmbH, Munich, Germany
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\AND
	\name Johannes Paetzold \\
	\addr
	Department of Informatics, Technical University Munich, Germany \\
	%
	\addr
	Helmholtz Zentrum München, Germany \\
	%
	\addr
	Imperial College London, Exhibition Rd, South Kensington, London SW7 2BX, United Kingdom
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\AND
	\name Hongwei Li \\
	\addr
	Department of Informatics, Technical University Munich, Germany \\
	%
	\addr
	Department of Quantitative Biomedicine, University of Zurich, Switzerland
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\AND
	\name Suprosanna Shit \\
	\addr
	Department of Informatics, Technical University Munich, Germany \\
	% 
	\addr 
	TranslaTUM - Central Institute for Translational Cancer Research, Technical University of Munich, Germany
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\AND
	\name Richard McKinley \\
	\addr
	Support Center for Advanced Neuroimaging (SCAN), University Institute of Diagnostic and Interventional Neuroradiology, University of Bern, Inselspital, Bern University Hospital, Bern, Switzerland
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\AND
	\name Marie Piraud \\
	\addr
	Helmholtz AI, Helmholtz Zentrum München, Germany
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\AND
	\name Spyridon Bakas \\
	\addr
	Center for Biomedical Image Computing and Analytics (CBICA), University of Pennsylvania, Philadelphia, Pennsylvania, USA \\
	%
	\addr
	Department of Pathology and Laboratory Medicine, Perelman School of Medicine, University of Pennsylvania, Philadelphia, Pennsylvania, USA \\
	%
	\addr
	Department of Radiology, Perelman School of Medicine, University of Pennsylvania, Philadelphia, Pennsylvania, USA
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\AND
	\name Claus Zimmer  \\
	\addr
	Department of Diagnostic and Interventional Neuroradiology, School of Medicine, Klinikum rechts der Isar, Technical University of Munich, Germany
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\AND
	\name Nassir Navab \\
	\addr
	Computer Aided Medical Procedures (CAMP), Technical University of Munich, Germany
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\AND
	\name Jan Kirschke \\
	\addr
	Department of Diagnostic and Interventional Neuroradiology, School of Medicine, Klinikum rechts der Isar, Technical University of Munich, Germany
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\AND
	\name Benedikt Wiestler \\
	\addr
	Department of Diagnostic and Interventional Neuroradiology, School of Medicine, Klinikum rechts der Isar, Technical University of Munich, Germany
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\AND
	\name Bjoern Menze \\
	\addr
	Department of Informatics, Technical University Munich, Germany \\
	%
	\addr
	Department of Quantitative Biomedicine, University of Zurich, Switzerland
}


==> flow/front/_old_authors.tex <==
% \author{First Author\\
% Institution1\\
% Institution1 address\\
% {\tt\small firstauthor@i1.org}
% % For a paper whose authors are all at the same institution,
% % omit the following lines up until the closing ``}''.
% % Additional authors and addresses can be added with ``\and'',
% % just like the second author.
% % To save space, use either the email address or home page, not both
% \and
% Second Author\\
% Institution2\\
% First line of institution2 address\\
% {\tt\small secondauthor@i2.org}
% }


\newcommand*\samethanks[1][\value{footnote}]{\footnotemark[#1]}

\author{Florian Kofler\inst{1,7,8} \and
Ivan Ezhov\inst{1,8} \and
Fabian Isensee \inst{2} \and
Fabian Balsiger \inst{3} \and
Christoph Berger \inst{1} \and
Maximilian Koerner \inst{1} \and
Beatrice Demiray \inst{1} \and
Julia Rackerseder \inst{1} \and
Johannes Paetzold \inst{1,8} \and
Hongwei Li \inst{1,10} \and
Suprosanna Shit \inst{1,8} \and
Richard McKinley \inst{3} \and
Spyridon Bakas \inst{4,5,6} \and
Claus Zimmer \inst{7} \and
Donna Ankerst \inst{9} \and
Nassir Navab \inst{1,11} \and
Jan Kirschke \inst{7,8} \and
Benedikt Wiestler\inst{7,8}\thanks{contributed equally as senior authors} \and
Bjoern H. Menze\inst{1,10}\samethanks}
%

% \authorrunning{F. Kofler et al.}
% % First names are abbreviated in the running head.
% % If there are more than two authors, 'et al.' is used.
% %
\institute{Department of Informatics, Technical University Munich, Germany\and 
HIP Applied Computer Vision Lab, Division of Medical Image Computing, German Cancer Research Center (DKFZ), Germany\and
Support Center for Advanced Neuroimaging (SCAN), Institute for Diagnostic and Interventional Neuroradiology, Inselspital, Bern University Hospital, University of Bern, Switzerland\and
Center for Biomedical Image Computing and Analytics (CBICA), University of Pennsylvania, USA\and
Department of Radiology, Perelman School of Medicine, University of Pennsylvania, USA\and
Department of Pathology and Laboratory Medicine, Perelman School of Medicine, University of Pennsylvania, USA\and
Department of Diagnostic and Interventional Neuroradiology, School of Medicine, Klinikum rechts der Isar, Technical University of Munich, Germany\and
TranslaTUM - Central Institute for Translational Cancer Research, Technical University of Munich, Germany\and
Depts of Mathematics and Life Science Systems, Technical University of Munich, Germany \and
Department of Quantitative Biomedicine, University of Zurich, Switzerland \and
Johns Hopkins University, Baltimore, USA
\\
\email{\{florian.kofler\}@tum.de}}



% florian.kofler@tum.de
% ivan.ezhov@tum.de
% lucas.fidon@kcl.ac.uk
% ezequiel.delarosa@icometrix.com


% johannes.paetzold@tum.de
% hongwei.li@tum.de
% izabela.horvath@tum.de
% suprosanna.shit@tum.de
% tom.finck@tum.de


% seniors
% sbakas@upenn.edu
% marie.piraud@helmholtz-muenchen.de 
% jan.kirschke@tum.de
% tom.vercauteren@kcl.ac.uk 
% claus.zimmer@tum.de
% b.wiestler@tum.de
% bjoern.menze@tum.de






blob loss:
% author emails (no particular order)
% florian.kofler@tum.de
% suprosanna.shit@tum.de
% ivan.ezhov@tum.de
% lucas.fidon@kcl.ac.uk
% izabela.horvath@tum.de

% rami.al-maskari@tum.de
% hongwei.li@tum.de

% harsharan.bhatia@med.uni-muenchen.de
% timo.loehr@tum.de

% erturk@helmholtz-muenchen.de
% jan.kirschke@tum.de
% jan.peeken@tum.de
% tom.vercauteren@kcl.ac.uk 
% claus.zimmer@tum.de
% b.wiestler@tum.de
% bjoern.menze@tum.de


ICML:
% author emails
% florian.kofler@tum.de
% ivan.ezhov@tum.de
% f.isensee@dkfz-heidelberg.de
% fabian.balsiger@insel.ch
% c.berger@tum.de
% maximilian.koerner@gmx.com
% beatrice.demiray@tum.de
% julia.rackerseder@mail.de
% johannes.paetzold@tum.de
% hongwei.li@tum.de
% suprosanna.shit@tum.de
% richard.mckinley@insel.ch
% marie.piraud@helmholtz-muenchen.de 
% sbakas@upenn.edu
% claus.zimmer@tum.de
% ankerst@tum.de
% nassir.navab@tum.de
% jan.kirschke@tum.de
% b.wiestler@tum.de
% bjoern.menze@tum.de





